PeopleSansPeople: A Synthetic Data Generator for Human-Centric Computer Vision

In recent years, person detection and human pose estimation have made great strides, helped by large-scale labeled datasets. However, these datasets had no guarantees or analysis of human activities, poses, or context diversity. Additionally, privacy, legal, safety, and ethical concerns may limit the ability to collect more human data. An emerging alternative to real-world data that alleviates some of these issues is synthetic data. However, creation of synthetic data generators is incredibly challenging and prevents researchers from exploring their usefulness. Therefore, we release a human-centric synthetic data generator PeopleSansPeople which contains simulation-ready 3D human assets, a parameterized lighting and camera system, and generates 2D and 3D bounding box, instance and semantic segmentation, and COCO pose labels. Using PeopleSansPeople, we performed benchmark synthetic data training using a Detectron2 Keypoint R-CNN variant [1]. We found that pre-training a network using synthetic data and fine-tuning on various sizes of real-world data resulted in a keypoint AP increase of $+38.03$ ($44.43 \pm 0.17$ vs. $6.40$) for few-shot transfer (limited subsets of COCO-person train [2]), and an increase of $+1.47$ ($63.47 \pm 0.19$ vs. $62.00$) for abundant real data regimes, outperforming models trained with the same real data alone. We also found that our models outperformed those pre-trained with ImageNet with a keypoint AP increase of $+22.53$ ($44.43 \pm 0.17$ vs. $21.90$) for few-shot transfer and $+1.07$ ($63.47 \pm 0.19$ vs. $62.40$) for abundant real data regimes. This freely-available data generator should enable a wide range of research into the emerging field of simulation to real transfer learning in the critical area of human-centric computer vision.

==> scraps/results_20210819.tex <==
% ===============================================================================================
% ===============================================================================================
% ===============================================================================================
\section{Results}
\label{results}
% Detectron2 COCO Person Keypoint Detection Baselines with Keypoint R-CNN R50-FPN 3x lr schedule:
% box AP: 55.4
% kp. AP: 65.5
% STEPS: (210000, 250000)
% MAXITER: 270000

\subsection{Training from scratch}
To obtain some healthy baselines, we train the Detectron2 Keypoint R-CNN \texttt{R50-FPN} model from scratch with the strategies described in Section \ref{subsection:training} using limited and abundant real data, and various sizes of synthetic data for person bounding box (bbox) and keypoint detection. We do so, as in \citep{he2019rethinking} the authors posited that ``training from scratch will yield no worse results than pre-training on ImageNet'', under limited and abundant data regiments. Based on this argument, which is backed up by ample evidence, we base our analysis on benchmarks obtained from models trained from scratch under many circumstances.
We report our results in the form of COCO metrics and use Average Precision (AP) as the main metric for model performance. 

In the case of training on real data, we discover that the model performance tends to increase rapidly when the size of the data is increased, and then tends to saturate when there is plentiful data as can be seen in Table \ref{tab:scratch_results}. To sanity-check our results, we also reconfirm the findings of \citep{he2019rethinking} that models trained from scratch on ample data can indeed catch up in accuracy with models that are fine-tuned after pre-training on ImageNet. The model trained on the entire COCO person dataset achieves a keypoint AP of $65.12$ and bounding box AP of $56.73$, while the same model pre-trained on ImageNet and then fine-tuned on COCO is reported to achieve a keypoint AP of $65.5$ and bounding box AP of $55.4$ by Detectron2 \citep{he2019rethinking}.

We train the model from scratch on varying sizes of synthetic dataset too and report the validation performance on COCO person validation set in Table \ref{tab:scratch_results}. The results indicate that a model trained solely on our na\"ively-generated synthetic data struggles to generalize on the real domain, and no amount of synthetic data seems to help with this.

\subsection{Transfer-Learning From Synthetic Pre-Training}
We take the models trained from scratch on synthetic data that we described in the previous section and fine-tune them on limited and abundant real data. We use the term ``transfer-learning'' for this fine-tuning operation, since we are transferring model weights from the synthetic (simulation) to the real domain. We find surprisingly that the pre-training on the synthetic data does indeed help boost model performance after fine-tuning with limited and abundant data. Interestingly, we observe larger impact as the size of the synthetic data used for pre-training is increased, with some diminishing returns beyond a certain synthetic data size as shown in Table \ref{tab:transfer_results} and Figure \ref{fig:kpt}. As mentioned in Section \ref{subsection:training} we cap the number of iterations for training all models at $1M$. Consequently the models trained with $245K$ and $490K$ synthetic data are not trained until the learning rate has been reduced three times. We expect the results for these models to improve when the training is performed for much longer than $1M$ iterations.

Our best models pre-trained on synthetic data and fine-tuned on the entire COCO achieve a keypoint AP of $66.62$ and bounding box AP of $57.51$, outperforming the same model only trained on COCO from scratch which achieves a keypoint AP of $65.12$ and bounding box AP of $56.73$. 

\subsection{Discussion}
\sujoy{Comment from Salehe: Please comment the observations as opposed to deleting them, in case you'd like to cut some off the paper. I want to have these on record here for future food for thought or research ideas.}

It is worth noting that we did not perform any grid search for hyper-parameters in any of our model training experiments; neither did we vary model seed, initialization, or model configuration. The length of training is only governed by the size of the dataset and performance on the validation set as described before in Section \ref{subsection:training} to provide all the models with the same training regiment under the same recipe. These results indicate that our methodology of adopting the same optimization strategy with no changes to the rest of the parameters, will only reflect the effect of the data size and pre-training on synthetic data on model performance. To this end, we have demonstrated the efficacy of our synthetic data generator in enabling better generalization in human-centric computer vision using an ``off-the-shelf'' model architecture. In summary we observed that:

\paragraph{Training from scratch yields inferior results with limited and abundant real data.} The synthetic data pre-training helps boost the performance even though the synthetic data itself was not fine-tuned to do so.

\paragraph{There exists a domain gap between our synthetic data and the real data, although there is promise to be discovered for addressing this.} Our models trained only on synthetic data from scratch perform poorly on real data as shown in Table \ref{tab:scratch_results}. However, we do observe some variation in the performance. The synthetic data generator comes with highly-parameterized randomizers and knobs to tweak and turn. It is also possible for the users to easily integrate their own randomizers into our data generator. Therefore, it is a reasonable assumption that tweaking and turning these knobs the \textit{``right''} way will positively impact model performance.

\paragraph{Fine-tuning on real data from pre-trained synthetic weights requires variable iterations to sufficiently converge.} This is shown in the checkpoints column in Table \ref{tab:transfer_results}, where we have three generator seeds for each size of synthetic data. The large variations in the checkpoint numbers over the same dataset size and across multiple dataset seeds indicate that there might be some \textit{``right''} set of synthetic data that will be sufficient for training a model faster.

\paragraph{We find that synthetic data pre-training does not necessarily help reduce over-fitting except for the limited data regime.} In the case of using $1\%$ and $10\%$ of COCO ($641$ and $6411$ images respectively), we observe the largest effect of pre-training on synthetic in Table \ref{tab:transfer_results}. We list the largest gains in Table \ref{tab:delta_ap}.

\paragraph{Training from scratch is inferior to pre-training on synthetic data for domain-specific tasks.} In \citep{he2019rethinking} the authors prescribed that ``training from scratch can be no worse than its ImageNet pre-training counterparts''; while this is true when the pre-training dataset is thought of as a universal generalist, we find that this is not true -- as far as our experiments set is concerned -- at least for domain-specific task of person bounding box and keypoint detection. Therefore, for domain-specific computer vision, synthetic data \textit{may} provide a better auxiliary role than ImageNet pre-training.

\paragraph{Synthetic pre-training helps more with localization of keypoints than bounding box detection.} In Table \ref{tab:delta_ap} we show the gains of synthetic pre-training over training from scratch for the best models. The gains are indeed larger for keypoint localization than classification of a region of the image.

\subsection{Future Research Directions}
With the encouraging results in our transfer-learning experiments, we leave open further research into hyper-parameter search, optimization strategy, and training scheduling for ourselves and the readers. Furthermore, there might be better alternatives than pre-training on synthetic and fine-tuning on real data, such as dataset mixing with interleaved or balanced sets, or alternating between synthetic and real training. Our synthetic data generator can also facilitate meta-learning approaches where data generation is a function of model performance in a feedback loop. We envisage that the most interesting line of research would involve generating synthetic data that bridges the simulation to real transfer learning and addresses the domain gap between the synthetic and the real data; something that we observed in our training from scratch experiments when synthetically trained models were not able to generalize well when presented with real-world data. We anticipate that our highly-parameterized domain randomization regiment can expedite this type of research. Our data generator also facilitates other human-centric computer vision research, such as semantic and instance segmentation and 3D bounding box localization.

\input{tables/table_scratch_results}

\input{tables/table_transfer_results}

\input{tables/table_gains}

\begin{figure}[]
\centering
\includegraphics[width=0.6\textwidth, trim={0.85cm 0.15cm 1.3cm 1.75cm},clip]{neurips_data_2021/plots/results_fig/kpt_ap_transfer_size_linear.pdf}
% \subfloat[\centering]{\fbox{{\includegraphics[width=0.45\textwidth, trim={0.75cm 0.2cm 1.75cm 0.65cm},clip]{neurips_data_2021/plots/results_fig/kpt_ap_transfer_size_linear.pdf} }}}%
% \qquad
% \subfloat[\centering]{\fbox{{\includegraphics[width=0.45\textwidth, trim={0.75cm 0.2cm 1.75cm 0.65cm},clip]{neurips_data_2021/plots/results_fig/kpt_ap_transfer_size_symlog.pdf} }}}%
\caption{\textbf{The keypoint Average Precision (AP) over different sizes of synthetic and real-world datasets.} 
For the blue curve, we report the evaluation results of synthetic pre-trained models on COCO validation set.
The other curves each show a different size of real-world dataset used to fine-tune from pre-trained synthetic weights. The points on each curve delineate different sizes of synthetic datasets ($0$, $4.9K$, $49K$, $245K$, and $490K$ respectively, where $0$ synthetic data is the result of training from scratch on real data only).}
\label{fig:kpt}
\end{figure}



==> scraps/xx_Sidewaystable.tex <==
% \begin{table}[]
% \caption{Training from scratch results. Normal table.}
% \begin{adjustbox}{max width=\textwidth}
% \centering
% \begin{tabular}{lrrcccccc}
% \toprule
%               &      &                          & \multicolumn{6}{c}{bbox} \\
% \cmidrule(lr){4-9}
%              dataset &     dataset size &                         checkpoints &               AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$ &              $\textrm{AP}^{\textrm{\textit{small}}}$ \\
% \midrule
% COCO dataset & 641 &                       5280 &            13.82 &             36.49 &             7.01 &             21.98 &            17.64 &             6.83 \\
%               & 6411 &                      40000 &            37.82 &             69.08 &            37.18 &             54.14 &            44.22 &            22.21 \\
%               & 32057 &                     168252 &            52.15 &             81.89 &            56.09 &             68.84 &            58.78 &            35.09 \\
%               & 64115 &                     577008 &            56.73 &             85.20 &            61.49 &             73.23 &            63.56 &            39.14 \\\\
% Synth dataset & 4.9K &      [38556, 53244, 38556] &  4.34 $\pm$ 0.12 &   8.46 $\pm$ 0.29 &  3.82 $\pm$ 0.11 &   8.61 $\pm$ 0.20 &  5.94 $\pm$ 0.02 &  1.29 $\pm$ 0.13 \\
%               & 49K &   [391936, 594028, 398060] &  7.61 $\pm$ 0.12 &  14.65 $\pm$ 0.33 &  7.00 $\pm$ 0.09 &  14.48 $\pm$ 1.30 &  9.86 $\pm$ 0.27 &  2.36 $\pm$ 0.10 \\
%               & 245K &  [979968, 979968, 1010592] &  5.70 $\pm$ 0.99 &  11.03 $\pm$ 2.36 &  5.15 $\pm$ 0.62 &  11.45 $\pm$ 1.05 &  7.68 $\pm$ 1.12 &  2.15 $\pm$ 0.31 \\
%               & 490K &  [857500, 1041250, 980000] &  6.14 $\pm$ 0.71 &  11.71 $\pm$ 1.31 &  5.58 $\pm$ 0.77 &  12.15 $\pm$ 2.09 &  8.35 $\pm$ 0.65 &  1.87 $\pm$ 0.30 \\\\
% \toprule
%               &      &                          & \multicolumn{6}{c}{keypoint} \\
% \cmidrule(lr){4-9}              
%               dataset &     dataset size &                         checkpoints &               AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$ &               \\
% \midrule
% COCO dataset & 641 &                       5280 &             7.47 &             23.26 &             3.10 &              8.85 &             6.88 &                  \\
%               & 6411 &                      40000 &            39.48 &             69.04 &            38.66 &             44.87 &            36.36 &                  \\
%               & 32057 &                     168252 &            58.68 &             83.51 &            63.10 &             65.41 &            55.15 &                  \\
%               & 64115 &                     577008 &            65.12 &             86.73 &            70.97 &             72.64 &            61.15 &                  \\\\
% Synth dataset & 4.9K &      [38556, 53244, 38556] &  1.89 $\pm$ 0.29 &   4.64 $\pm$ 0.31 &  1.26 $\pm$ 0.29 &   1.92 $\pm$ 0.30 &  2.22 $\pm$ 0.15 &                  \\
%               & 49K &   [391936, 594028, 398060] &  5.47 $\pm$ 0.10 &  11.77 $\pm$ 0.28 &  4.54 $\pm$ 0.19 &   5.50 $\pm$ 0.44 &  6.42 $\pm$ 0.16 &                  \\
%               & 245K &  [979968, 979968, 1010592] &  3.49 $\pm$ 0.33 &   7.20 $\pm$ 0.82 &  2.90 $\pm$ 0.31 &   3.74 $\pm$ 0.76 &  4.53 $\pm$ 0.56 &                  \\
%               & 490K &  [857500, 1041250, 980000] &  4.25 $\pm$ 0.53 &   9.07 $\pm$ 1.11 &  3.36 $\pm$ 0.51 &   4.42 $\pm$ 0.95 &  5.07 $\pm$ 0.41 &                  \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% % \caption{Caption}
% \label{tab:my_label}
% \end{table}


% \begin{table}[]
% \caption{Transfer learning with real data from pre-trained synthetic weights. Normal Table}
% \begin{adjustbox}{max width=\textwidth}
% \centering
% \begin{tabular}{rrrcccccc}
% \toprule
%     %   &      &                        ck & \multicolumn{6}{l}{val real} \\
%       &      &                         & \multicolumn{6}{c}{bbox} \\
% \cmidrule(lr){4-9}      
%      size of real data &     size of synth data &               checkpoints &                AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$ &              $\textrm{AP}^{\textrm{\textit{small}}}$ \\
% \midrule
% 641 & 0 &                      5280 &             13.82 &             36.49 &              7.01 &             21.98 &             17.64 &              6.83 \\
%       & 4.9K &        [2960, 2240, 3840] &  30.32 $\pm$ 0.48 &  56.58 $\pm$ 0.75 &  28.90 $\pm$ 0.53 &  43.86 $\pm$ 0.36 &  37.00 $\pm$ 0.47 &  16.47 $\pm$ 0.51 \\
%       & 49K &          [880, 720, 2480] &  39.65 $\pm$ 0.64 &  66.92 $\pm$ 1.03 &  40.36 $\pm$ 0.74 &  54.16 $\pm$ 0.52 &  47.74 $\pm$ 0.73 &  23.65 $\pm$ 0.92 \\
%       & 245K &           [640, 880, 800] &  40.68 $\pm$ 0.32 &  68.14 $\pm$ 0.54 &  41.79 $\pm$ 0.39 &  55.42 $\pm$ 0.07 &  48.76 $\pm$ 0.19 &  24.79 $\pm$ 0.68 \\
%       & 490K &          [960, 800, 1360] &  40.70 $\pm$ 0.60 &  68.26 $\pm$ 0.83 &  41.34 $\pm$ 0.84 &  55.32 $\pm$ 0.62 &  48.87 $\pm$ 0.41 &  24.79 $\pm$ 0.79 \\\\
% 6411 & 0 &                     40000 &             37.82 &             69.08 &             37.18 &             54.14 &             44.22 &             22.21 \\
%       & 4.9K &     [27200, 15200, 21600] &  42.83 $\pm$ 0.37 &  72.85 $\pm$ 0.24 &  44.01 $\pm$ 0.37 &  58.93 $\pm$ 0.37 &  49.92 $\pm$ 0.39 &  26.34 $\pm$ 0.59 \\
%       & 49K &     [13600, 13600, 14400] &  48.46 $\pm$ 0.29 &  77.48 $\pm$ 0.21 &  51.22 $\pm$ 0.45 &  64.18 $\pm$ 0.37 &  56.00 $\pm$ 0.13 &  31.38 $\pm$ 0.58 \\
%       & 245K &     [12000, 15200, 19200] &  49.79 $\pm$ 0.13 &  78.61 $\pm$ 0.08 &  52.75 $\pm$ 0.32 &  65.78 $\pm$ 0.11 &  57.50 $\pm$ 0.27 &  32.10 $\pm$ 0.15 \\
%       & 490K &      [8800, 13600, 13600] &  49.63 $\pm$ 0.20 &  78.55 $\pm$ 0.09 &  52.60 $\pm$ 0.37 &  65.32 $\pm$ 0.15 &  57.25 $\pm$ 0.25 &  32.30 $\pm$ 0.37 \\\\
% 32057 & 0 &                    168252 &             52.15 &             81.89 &             56.09 &             68.84 &             58.78 &             35.09 \\
%       & 4.9K &  [168252, 184276, 200300] &  52.97 $\pm$ 0.04 &  82.20 $\pm$ 0.04 &  56.95 $\pm$ 0.04 &  69.69 $\pm$ 0.05 &  59.83 $\pm$ 0.16 &  35.56 $\pm$ 0.17 \\
%       & 49K &   [100150, 96144, 100150] &  54.74 $\pm$ 0.20 &  83.38 $\pm$ 0.06 &  59.22 $\pm$ 0.25 &  71.31 $\pm$ 0.34 &  61.51 $\pm$ 0.04 &  37.20 $\pm$ 0.15 \\
%       & 245K &   [80120, 108162, 112168] &  55.05 $\pm$ 0.08 &  83.60 $\pm$ 0.10 &  59.28 $\pm$ 0.11 &  71.58 $\pm$ 0.22 &  61.90 $\pm$ 0.08 &  37.36 $\pm$ 0.33 \\
%       & 490K &  [100150, 104156, 128192] &  55.01 $\pm$ 0.19 &  83.60 $\pm$ 0.10 &  59.48 $\pm$ 0.42 &  71.45 $\pm$ 0.19 &  61.95 $\pm$ 0.11 &  37.16 $\pm$ 0.31 \\\\
% 64115 & 0 &                    577008 &             56.73 &             85.20 &             61.49 &             73.23 &             63.56 &             39.14 \\
%       & 4.9K &  [416728, 432756, 472826] &  56.65 $\pm$ 0.02 &  85.15 $\pm$ 0.02 &  61.62 $\pm$ 0.30 &  73.07 $\pm$ 0.16 &  63.46 $\pm$ 0.06 &  39.19 $\pm$ 0.12 \\
%       & 49K &  [384672, 400700, 376658] &  57.24 $\pm$ 0.06 &  85.34 $\pm$ 0.11 &  62.36 $\pm$ 0.18 &  73.79 $\pm$ 0.31 &  64.04 $\pm$ 0.05 &  39.66 $\pm$ 0.19 \\
%       & 245K &  [304532, 400700, 256448] &  57.39 $\pm$ 0.11 &  85.41 $\pm$ 0.06 &  62.47 $\pm$ 0.22 &  73.98 $\pm$ 0.09 &  64.31 $\pm$ 0.13 &  39.46 $\pm$ 0.18 \\
%       & 490K &  [240420, 376658, 328574] &  57.51 $\pm$ 0.26 &  85.68 $\pm$ 0.31 &  62.62 $\pm$ 0.36 &  73.95 $\pm$ 0.20 &  64.42 $\pm$ 0.20 &  39.64 $\pm$ 0.27 \\\\
% \toprule
%     %   &      &                        ck & \multicolumn{6}{l}{val real} \\
%       &      &                         & \multicolumn{6}{c}{keypoint} \\
% \cmidrule(lr){4-9}      
%      size of real data &     size of synth data &               checkpoints &                AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$ &               \\
% \midrule     
% 641 & 0 &                      5280 &              7.47 &             23.26 &              3.10 &              8.85 &              6.88 &                   \\
%       & 4.9K &        [2960, 2240, 3840] &  25.02 $\pm$ 0.53 &  53.20 $\pm$ 0.65 &  20.14 $\pm$ 0.77 &  27.13 $\pm$ 0.48 &  24.05 $\pm$ 0.55 &                   \\
%       & 49K &          [880, 720, 2480] &  41.53 $\pm$ 1.46 &  69.03 $\pm$ 1.17 &  41.95 $\pm$ 1.84 &  44.52 $\pm$ 1.20 &  40.28 $\pm$ 1.69 &                   \\
%       & 245K &           [640, 880, 800] &  44.49 $\pm$ 0.23 &  71.45 $\pm$ 0.56 &  45.62 $\pm$ 0.30 &  48.29 $\pm$ 0.31 &  42.73 $\pm$ 0.18 &                   \\
%       & 490K &          [960, 800, 1360] &  44.69 $\pm$ 0.10 &  71.42 $\pm$ 0.14 &  45.99 $\pm$ 0.15 &  48.30 $\pm$ 0.32 &  43.08 $\pm$ 0.11 &                   \\\\
% 6411 & 0 &                     40000 &             39.48 &             69.04 &             38.66 &             44.87 &             36.36 &                   \\
%       & 4.9K &     [27200, 15200, 21600] &  44.22 $\pm$ 0.39 &  72.84 $\pm$ 0.41 &  45.36 $\pm$ 0.53 &  49.75 $\pm$ 0.36 &  41.35 $\pm$ 0.59 &                   \\
%       & 49K &     [13600, 13600, 14400] &  53.23 $\pm$ 0.55 &  79.36 $\pm$ 0.44 &  56.69 $\pm$ 0.46 &  58.83 $\pm$ 0.43 &  50.37 $\pm$ 0.64 &                   \\
%       & 245K &     [12000, 15200, 19200] &  55.98 $\pm$ 0.38 &  81.34 $\pm$ 0.18 &  60.50 $\pm$ 0.39 &  61.78 $\pm$ 0.26 &  53.11 $\pm$ 0.43 &                   \\
%       & 490K &      [8800, 13600, 13600] &  55.82 $\pm$ 0.20 &  81.11 $\pm$ 0.37 &  60.12 $\pm$ 0.36 &  61.49 $\pm$ 0.21 &  52.94 $\pm$ 0.32 &                   \\\\
% 32057 & 0 &                    168252 &             58.68 &             83.51 &             63.10 &             65.41 &             55.15 &                   \\
%       & 4.9K &  [168252, 184276, 200300] &  58.91 $\pm$ 0.21 &  83.63 $\pm$ 0.09 &  63.65 $\pm$ 0.38 &  66.07 $\pm$ 0.30 &  54.99 $\pm$ 0.30 &                   \\
%       & 49K &   [100150, 96144, 100150] &  62.29 $\pm$ 0.23 &  85.19 $\pm$ 0.17 &  67.79 $\pm$ 0.19 &  69.42 $\pm$ 0.32 &  58.42 $\pm$ 0.35 &                   \\
%       & 245K &   [80120, 108162, 112168] &  63.13 $\pm$ 0.25 &  86.04 $\pm$ 0.14 &  68.89 $\pm$ 0.12 &  70.15 $\pm$ 0.14 &  59.28 $\pm$ 0.37 &                   \\
%       & 490K &  [100150, 104156, 128192] &  62.92 $\pm$ 0.34 &  85.77 $\pm$ 0.39 &  68.29 $\pm$ 0.43 &  69.89 $\pm$ 0.43 &  59.10 $\pm$ 0.32 &                   \\\\
% 64115 & 0 &                    577008 &             65.12 &             86.73 &             70.97 &             72.64 &             61.15 &                   \\
%       & 4.9K &  [416728, 432756, 472826] &  65.19 $\pm$ 0.12 &  87.28 $\pm$ 0.01 &  70.79 $\pm$ 0.42 &  72.52 $\pm$ 0.31 &  61.24 $\pm$ 0.11 &                   \\
%       & 49K &  [384672, 400700, 376658] &  65.81 $\pm$ 0.19 &  87.39 $\pm$ 0.32 &  71.81 $\pm$ 0.43 &  73.20 $\pm$ 0.05 &  61.76 $\pm$ 0.29 &                   \\
%       & 245K &  [304532, 400700, 256448] &  66.62 $\pm$ 0.32 &  87.78 $\pm$ 0.18 &  72.49 $\pm$ 0.24 &  73.76 $\pm$ 0.18 &  62.80 $\pm$ 0.44 &                   \\
%       & 490K &  [240420, 376658, 328574] &  66.48 $\pm$ 0.19 &  87.75 $\pm$ 0.06 &  72.16 $\pm$ 0.30 &  73.62 $\pm$ 0.35 &  62.54 $\pm$ 0.25 &                   \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% % \caption{Caption}
% \label{tab:my_label}
% \end{table}


\begin{sidewaystable}%[htbp]
\tiny
\centering
\caption{Training from scratch results. Sidewaystable.}
\begin{tabular*}{0.97\textwidth}{lrrccccccccccc}%{llllllllllllll}%{llrrrrrrrrrrrr}
\toprule
    %   &            &      & \multicolumn{11}{c}{val real} \\
       &            &        & \multicolumn{5}{c}{keypoint} & \multicolumn{6}{c}{bbox} \\
       \cmidrule(lr){4-8}\cmidrule(lr){9-14}
      dataset &           dataset size &       checkpoint &       AP &   $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &   $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &    $\textrm{AP}^{\textrm{\textit{large}}}$ &    $\textrm{AP}^{\textrm{\textit{medium}}}$ &     AP &   $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &   $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &    $\textrm{AP}^{\textrm{\textit{large}}}$ &    $\textrm{AP}^{\textrm{\textit{medium}}}$ &    $\textrm{AP}^{\textrm{\textit{small}}}$ \\
\midrule
COCO dataset & 641 &                       5280 &             7.47 &             23.26 &             3.10 &             8.85 &             6.88 &            13.82 &             36.49 &             7.01 &             21.98 &            17.64 &             6.83 \\
              & 6411 &                      40000 &            39.48 &             69.04 &            38.66 &            44.87 &            36.36 &            37.82 &             69.08 &            37.18 &             54.14 &            44.22 &            22.21 \\
              & 32057 &                     168252 &            58.68 &             83.51 &            63.10 &            65.41 &            55.15 &            52.15 &             81.89 &            56.09 &             68.84 &            58.78 &            35.09 \\
              & 64115 &                     577008 &            65.12 &             86.73 &            70.97 &            72.64 &            61.15 &            56.73 &             85.20 &            61.49 &             73.23 &            63.56 &            39.14 \\\\
Synth dataset & 4.9K &      [38556, 53244, 38556] &  1.89 $\pm$ 0.29 &   4.64 $\pm$ 0.31 &  1.26 $\pm$ 0.29 &  1.92 $\pm$ 0.30 &  2.22 $\pm$ 0.15 &  4.34 $\pm$ 0.12 &   8.46 $\pm$ 0.29 &  3.82 $\pm$ 0.11 &   8.61 $\pm$ 0.20 &  5.94 $\pm$ 0.02 &  1.29 $\pm$ 0.13 \\
              & 49K &   [391936, 594028, 398060] &  5.47 $\pm$ 0.10 &  11.77 $\pm$ 0.28 &  4.54 $\pm$ 0.19 &  5.50 $\pm$ 0.44 &  6.42 $\pm$ 0.16 &  7.61 $\pm$ 0.12 &  14.65 $\pm$ 0.33 &  7.00 $\pm$ 0.09 &  14.48 $\pm$ 1.30 &  9.86 $\pm$ 0.27 &  2.36 $\pm$ 0.10 \\
              & 245K &  [979968, 979968, 1010592] &  3.49 $\pm$ 0.33 &   7.20 $\pm$ 0.82 &  2.90 $\pm$ 0.31 &  3.74 $\pm$ 0.76 &  4.53 $\pm$ 0.56 &  5.70 $\pm$ 0.99 &  11.03 $\pm$ 2.36 &  5.15 $\pm$ 0.62 &  11.45 $\pm$ 1.05 &  7.68 $\pm$ 1.12 &  2.15 $\pm$ 0.31 \\
              & 490K &  [857500, 1041250, 980000] &  4.25 $\pm$ 0.53 &   9.07 $\pm$ 1.11 &  3.36 $\pm$ 0.51 &  4.42 $\pm$ 0.95 &  5.07 $\pm$ 0.41 &  6.14 $\pm$ 0.71 &  11.71 $\pm$ 1.31 &  5.58 $\pm$ 0.77 &  12.15 $\pm$ 2.09 &  8.35 $\pm$ 0.65 &  1.87 $\pm$ 0.30 \\
\bottomrule
\end{tabular*}
% \end{sidewaystable}
\bigskip\bigskip  % provide some separation between the two tables
% \begin{sidewaystable}
\tiny
\centering
\caption{Transfer learning with real data from pre-trained synthetic weights}
\begin{tabular*}{1.03\textwidth}{rrrccccccccccc}%{rrrlllllllllll}%{lllccccccccccc}
\toprule
        %  &            &                         & \multicolumn{11}{c}{real validation} \\
        %  \cmidrule(lr){4-14}
         &            &                         & \multicolumn{5}{c}{keypoint} & \multicolumn{6}{c}{bbox} \\
         \cmidrule(lr){4-8}\cmidrule(lr){9-14}
        size of real data &           size of synth data &               checkpoints &                AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &              $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &               $\textrm{AP}^{\textrm{\textit{medium}}}$ &                AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &              $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &               $\textrm{AP}^{\textrm{\textit{medium}}}$ &               $\textrm{AP}^{\textrm{\textit{small}}}$ \\
\midrule
641 & 0 &                      5280 &              7.47 &             23.26 &              3.10 &              8.85 &              6.88 &             13.82 &             36.49 &              7.01 &             21.98 &             17.64 &              6.83 \\
      & 4.9K &        [2960, 2240, 3840] &  25.02 $\pm$ 0.53 &  53.20 $\pm$ 0.65 &  20.14 $\pm$ 0.77 &  27.13 $\pm$ 0.48 &  24.05 $\pm$ 0.55 &  30.32 $\pm$ 0.48 &  56.58 $\pm$ 0.75 &  28.90 $\pm$ 0.53 &  43.86 $\pm$ 0.36 &  37.00 $\pm$ 0.47 &  16.47 $\pm$ 0.51 \\
      & 49K &          [880, 720, 2480] &  41.53 $\pm$ 1.46 &  69.03 $\pm$ 1.17 &  41.95 $\pm$ 1.84 &  44.52 $\pm$ 1.20 &  40.28 $\pm$ 1.69 &  39.65 $\pm$ 0.64 &  66.92 $\pm$ 1.03 &  40.36 $\pm$ 0.74 &  54.16 $\pm$ 0.52 &  47.74 $\pm$ 0.73 &  23.65 $\pm$ 0.92 \\
      & 245K &           [640, 880, 800] &  44.49 $\pm$ 0.23 &  71.45 $\pm$ 0.56 &  45.62 $\pm$ 0.30 &  48.29 $\pm$ 0.31 &  42.73 $\pm$ 0.18 &  40.68 $\pm$ 0.32 &  68.14 $\pm$ 0.54 &  41.79 $\pm$ 0.39 &  55.42 $\pm$ 0.07 &  48.76 $\pm$ 0.19 &  24.79 $\pm$ 0.68 \\
      & 490K &          [960, 800, 1360] &  44.69 $\pm$ 0.10 &  71.42 $\pm$ 0.14 &  45.99 $\pm$ 0.15 &  48.30 $\pm$ 0.32 &  43.08 $\pm$ 0.11 &  40.70 $\pm$ 0.60 &  68.26 $\pm$ 0.83 &  41.34 $\pm$ 0.84 &  55.32 $\pm$ 0.62 &  48.87 $\pm$ 0.41 &  24.79 $\pm$ 0.79 \\\\
6411 & 0 &                     40000 &             39.48 &             69.04 &             38.66 &             44.87 &             36.36 &             37.82 &             69.08 &             37.18 &             54.14 &             44.22 &             22.21 \\
      & 4.9K &     [27200, 15200, 21600] &  44.22 $\pm$ 0.39 &  72.84 $\pm$ 0.41 &  45.36 $\pm$ 0.53 &  49.75 $\pm$ 0.36 &  41.35 $\pm$ 0.59 &  42.83 $\pm$ 0.37 &  72.85 $\pm$ 0.24 &  44.01 $\pm$ 0.37 &  58.93 $\pm$ 0.37 &  49.92 $\pm$ 0.39 &  26.34 $\pm$ 0.59 \\
      & 49K &     [13600, 13600, 14400] &  53.23 $\pm$ 0.55 &  79.36 $\pm$ 0.44 &  56.69 $\pm$ 0.46 &  58.83 $\pm$ 0.43 &  50.37 $\pm$ 0.64 &  48.46 $\pm$ 0.29 &  77.48 $\pm$ 0.21 &  51.22 $\pm$ 0.45 &  64.18 $\pm$ 0.37 &  56.00 $\pm$ 0.13 &  31.38 $\pm$ 0.58 \\
      & 245K &     [12000, 15200, 19200] &  55.98 $\pm$ 0.38 &  81.34 $\pm$ 0.18 &  60.50 $\pm$ 0.39 &  61.78 $\pm$ 0.26 &  53.11 $\pm$ 0.43 &  49.79 $\pm$ 0.13 &  78.61 $\pm$ 0.08 &  52.75 $\pm$ 0.32 &  65.78 $\pm$ 0.11 &  57.50 $\pm$ 0.27 &  32.10 $\pm$ 0.15 \\
      & 490K &      [8800, 13600, 13600] &  55.82 $\pm$ 0.20 &  81.11 $\pm$ 0.37 &  60.12 $\pm$ 0.36 &  61.49 $\pm$ 0.21 &  52.94 $\pm$ 0.32 &  49.63 $\pm$ 0.20 &  78.55 $\pm$ 0.09 &  52.60 $\pm$ 0.37 &  65.32 $\pm$ 0.15 &  57.25 $\pm$ 0.25 &  32.30 $\pm$ 0.37 \\\\
32057 & 0 &                    168252 &             58.68 &             83.51 &             63.10 &             65.41 &             55.15 &             52.15 &             81.89 &             56.09 &             68.84 &             58.78 &             35.09 \\
      & 4.9K &  [168252, 184276, 200300] &  58.91 $\pm$ 0.21 &  83.63 $\pm$ 0.09 &  63.65 $\pm$ 0.38 &  66.07 $\pm$ 0.30 &  54.99 $\pm$ 0.30 &  52.97 $\pm$ 0.04 &  82.20 $\pm$ 0.04 &  56.95 $\pm$ 0.04 &  69.69 $\pm$ 0.05 &  59.83 $\pm$ 0.16 &  35.56 $\pm$ 0.17 \\
      & 49K &   [100150, 96144, 100150] &  62.29 $\pm$ 0.23 &  85.19 $\pm$ 0.17 &  67.79 $\pm$ 0.19 &  69.42 $\pm$ 0.32 &  58.42 $\pm$ 0.35 &  54.74 $\pm$ 0.20 &  83.38 $\pm$ 0.06 &  59.22 $\pm$ 0.25 &  71.31 $\pm$ 0.34 &  61.51 $\pm$ 0.04 &  37.20 $\pm$ 0.15 \\
      & 245K &   [80120, 108162, 112168] &  63.13 $\pm$ 0.25 &  86.04 $\pm$ 0.14 &  68.89 $\pm$ 0.12 &  70.15 $\pm$ 0.14 &  59.28 $\pm$ 0.37 &  55.05 $\pm$ 0.08 &  83.60 $\pm$ 0.10 &  59.28 $\pm$ 0.11 &  71.58 $\pm$ 0.22 &  61.90 $\pm$ 0.08 &  37.36 $\pm$ 0.33 \\
      & 490K &  [100150, 104156, 128192] &  62.92 $\pm$ 0.34 &  85.77 $\pm$ 0.39 &  68.29 $\pm$ 0.43 &  69.89 $\pm$ 0.43 &  59.10 $\pm$ 0.32 &  55.01 $\pm$ 0.19 &  83.60 $\pm$ 0.10 &  59.48 $\pm$ 0.42 &  71.45 $\pm$ 0.19 &  61.95 $\pm$ 0.11 &  37.16 $\pm$ 0.31 \\\\
64115 & 0 &                    577008 &             65.12 &             86.73 &             70.97 &             72.64 &             61.15 &             56.73 &             85.20 &             61.49 &             73.23 &             63.56 &             39.14 \\
      & 4.9K &  [416728, 432756, 472826] &  65.19 $\pm$ 0.12 &  87.28 $\pm$ 0.01 &  70.79 $\pm$ 0.42 &  72.52 $\pm$ 0.31 &  61.24 $\pm$ 0.11 &  56.65 $\pm$ 0.02 &  85.15 $\pm$ 0.02 &  61.62 $\pm$ 0.30 &  73.07 $\pm$ 0.16 &  63.46 $\pm$ 0.06 &  39.19 $\pm$ 0.12 \\
      & 49K &  [384672, 400700, 376658] &  65.81 $\pm$ 0.19 &  87.39 $\pm$ 0.32 &  71.81 $\pm$ 0.43 &  73.20 $\pm$ 0.05 &  61.76 $\pm$ 0.29 &  57.24 $\pm$ 0.06 &  85.34 $\pm$ 0.11 &  62.36 $\pm$ 0.18 &  73.79 $\pm$ 0.31 &  64.04 $\pm$ 0.05 &  39.66 $\pm$ 0.19 \\
      & 245K &  [304532, 400700, 256448] &  66.62 $\pm$ 0.32 &  87.78 $\pm$ 0.18 &  72.49 $\pm$ 0.24 &  73.76 $\pm$ 0.18 &  62.80 $\pm$ 0.44 &  57.39 $\pm$ 0.11 &  85.41 $\pm$ 0.06 &  62.47 $\pm$ 0.22 &  73.98 $\pm$ 0.09 &  64.31 $\pm$ 0.13 &  39.46 $\pm$ 0.18 \\
      & 490K &  [240420, 376658, 328574] &  66.48 $\pm$ 0.19 &  87.75 $\pm$ 0.06 &  72.16 $\pm$ 0.30 &  73.62 $\pm$ 0.35 &  62.54 $\pm$ 0.25 &  57.51 $\pm$ 0.26 &  85.68 $\pm$ 0.31 &  62.62 $\pm$ 0.36 &  73.95 $\pm$ 0.20 &  64.42 $\pm$ 0.20 &  39.64 $\pm$ 0.27 \\
\bottomrule
\end{tabular*}
\end{sidewaystable}

==> tables/table_bbox_size.tex <==
\begin{table}[htb]
\caption{Bounding box size.}
\begin{tabular}{lrrl}
Area Category & BBox Area Range         & COCO & Synth \\
Small         & {[}0 ** 2, 32 ** 2{]}   & 0.40 & 0.14  \\
Medium        & {[}32 ** 2, 96 ** 2{]}  & 0.34 & 0.48  \\
Large         & {[}96 ** 2, 1e5 ** 2{]} & 0.26 & 0.38 
\end{tabular}
\label{tab:bbox_size}
\end{table}

==> tables/table_gains.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\centering
\caption{\textbf{Comparison of gains obtained from pre-training on synthetic and fune-tuning on COCO over training from scratch on COCO.} For each dataset size we show the results of the best performing model from Table \ref{tab:transfer_results}.}
\label{tab:delta_ap}
\resizebox{0.58\textwidth}{!}{%
\begin{tabular}{rccr|ccr}
\toprule
 & \multicolumn{3}{c|}{bbox AP} & \multicolumn{3}{c}{keypoint AP} \\ 
 \midrule
\multicolumn{1}{r|}{size of real data} & scratch & w/ pre-train & $\Delta$ & scratch & w/ pre-train & $\Delta$ \\ 
\midrule
\multicolumn{1}{r|}{641} & 13.82 & 42.58 & +28.76 & 7.47 & 46.40 & +38.93 \\
\multicolumn{1}{r|}{6411} & 37.82 & 49.04 & +11.22 & 39.48 & 55.21 & +15.73 \\
\multicolumn{1}{r|}{32057} & 52.15 & 55.04 & +2.89 & 58.68 & 63.38 & +4.70 \\
\multicolumn{1}{r|}{64115} & 56.73 & 57.44 & +0.71 & 65.12 & 66.83 & +1.71 \\ 
\bottomrule
\end{tabular}%
}
\end{table}
% ===============================================================================================
% ====================================== OLD RESULTS ============================================
% ===============================================================================================
% \begin{table}[]
% \centering
% \caption{\sujoy{Old results with 1M iterations on 245K and 490K synth} \textbf{Comparison of gains obtained from pre-training on synthetic and fune-tuning on COCO over training from scratch on COCO.} For each dataset size we show the results of the best perfoming model from Table \ref{tab:transfer_results}.}
% \label{tab:delta_ap}
% \resizebox{0.58\textwidth}{!}{%
% \begin{tabular}{rccr|ccr}
% \toprule
%  & \multicolumn{3}{c|}{bbox AP} & \multicolumn{3}{c}{keypoint AP} \\ 
%  \midrule
% \multicolumn{1}{r|}{size of real data} & scratch & w/ pre-train & $\Delta$ & scratch & w/ pre-train & $\Delta$ \\ 
% \midrule
% \multicolumn{1}{r|}{641} & 13.82 & 40.70 & +26.88 & 7.47 & 44.69 & +37.22 \\
% \multicolumn{1}{r|}{6411} & 37.82 & 49.79 & +11.97 & 39.48 & 55.98 & +16.50 \\
% \multicolumn{1}{r|}{32057} & 52.15 & 55.05 & +2.90 & 58.68 & 63.13 & +4.45 \\
% \multicolumn{1}{r|}{64115} & 56.73 & 57.51 & +0.78 & 65.12 & 66.62 & +1.50 \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table}

==> tables/table_scratch_ood_crowdpose_results.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\caption{\textbf{Keypoint Metrics for Models Trained from Scratch - OOD Crowdpose Trainval.}
}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{lrrrccccc}
\toprule
              dataset &     dataset size &                         training steps & no. of epochs &               AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$                \\
\midrule
COCO & 641 &                         5280 &              132 &             9.12 &             27.58 &             4.14 &             9.97 &             6.49 \\
      & 6411 &                       168252 &               84 &            41.78 &             70.83 &            40.57 &            44.92 &            31.17 \\
      & 32057 &                        40000 &              100 &            62.44 &             84.22 &            65.91 &            65.97 &            49.13 \\
      & 64115 &                       577008 &              144 &            69.78 &             88.15 &            73.99 &            73.01 &            56.68 \\\\
Synth & $\text{4.9}\times10^3$ &        [38556, 53244, 38556] &  [126, 174, 126] &  2.25 $\pm$ 0.27 &   5.41 $\pm$ 0.52 &  1.52 $\pm$ 0.26 &  3.38 $\pm$ 0.25 &  1.01 $\pm$ 0.25 \\
      & $\text{49}\times10^3$ &     [391936, 594028, 398060] &  [128, 194, 130] &  5.08 $\pm$ 0.22 &  11.27 $\pm$ 0.63 &  3.78 $\pm$ 0.12 &  6.16 $\pm$ 0.48 &  3.46 $\pm$ 0.17 \\
      & $\text{245}\times10^3$ &  [2143680, 1745568, 2388672] &  [140, 114, 156] &  3.80 $\pm$ 0.12 &   7.83 $\pm$ 0.28 &  3.03 $\pm$ 0.09 &  4.38 $\pm$ 0.08 &  3.18 $\pm$ 0.17 \\
      & $\text{490}\times10^3$ &  [3920000, 4471250, 4042500] &  [128, 146, 132] &  3.48 $\pm$ 0.54 &   7.05 $\pm$ 1.19 &  2.82 $\pm$ 0.41 &  4.15 $\pm$ 0.70 &  2.62 $\pm$ 0.31 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:scratch_results_ood_crowdpose}
\end{table}


==> tables/table_scratch_ood_lspet_results.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\caption{\textbf{Keypoint Metrics for Models Trained from Scratch - OOD Leeds Sports.}
}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{lrrrccccc}
\toprule
              dataset &     dataset size &                         training steps & no. of epochs &               AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$                \\
\midrule
COCO & 641 &                         5280 &              132 &             1.19 &             4.43 &             0.33 &             2.51 &             0.62 \\
      & 6411 &                       168252 &               84 &             8.36 &            17.37 &             6.63 &            15.99 &             3.77 \\
      & 32057 &                        40000 &              100 &            18.43 &            30.72 &            18.22 &            29.24 &             8.73 \\
      & 64115 &                       577008 &              144 &            26.69 &            41.62 &            26.82 &            37.95 &            14.12 \\\\
Synth & $\text{4.9}\times10^3$ &        [38556, 53244, 38556] &  [126, 174, 126] &  0.65 $\pm$ 0.15 &  1.63 $\pm$ 0.19 &  0.50 $\pm$ 0.38 &  1.06 $\pm$ 0.10 &  0.60 $\pm$ 0.06 \\
      & $\text{49}\times10^3$ &     [391936, 594028, 398060] &  [128, 194, 130] &  0.60 $\pm$ 0.02 &  1.32 $\pm$ 0.13 &  0.50 $\pm$ 0.10 &  1.19 $\pm$ 0.17 &  0.13 $\pm$ 0.01 \\
      & $\text{245}\times10^3$ &  [2143680, 1745568, 2388672] &  [140, 114, 156] &  0.24 $\pm$ 0.02 &  0.44 $\pm$ 0.05 &  0.21 $\pm$ 0.03 &  0.60 $\pm$ 0.05 &  0.08 $\pm$ 0.02 \\
      & $\text{490}\times10^3$ &  [3920000, 4471250, 4042500] &  [128, 146, 132] &  0.33 $\pm$ 0.03 &  0.49 $\pm$ 0.07 &  0.39 $\pm$ 0.08 &  0.83 $\pm$ 0.05 &  0.05 $\pm$ 0.01 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:scratch_results_ood_lspet}
\end{table}


==> tables/table_scratch_ood_mpii_results.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\caption{\textbf{Keypoint Metrics for Models Trained from Scratch - OOD MPII Train.}
}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{lrrrccccc}
\toprule
              dataset &     dataset size &                         training steps & no. of epochs &               AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$                \\
\midrule
COCO & 641 &                         5280 & 132 &             13.99 &             37.63 &             7.90 &             14.62 &             1.24     \\
              & 6411 &                        40000 & 100 &             48.66 &             76.69 &            49.54 &             50.40 &             4.71     \\
              & 32057 &                       168252 & 84 &             66.86 &             86.97 &            72.77 &             68.27 &             8.65     \\
              & 64115 &                       577008 & 144 &             71.85 &             89.36 &            78.22 &             73.17 &            10.53     \\\\
Synth & $\text{4.9}\times10^3$ &        [38556, 53244, 38556] & [126, 174, 126] &   5.24 $\pm$ 0.47 &  11.10 $\pm$ 0.93 &  4.19 $\pm$ 0.44 &   6.49 $\pm$ 0.52 &  1.08 $\pm$ 0.47     \\
              & $\text{49}\times10^3$ &     [391936, 594028, 398060] & [128, 194, 130] &  10.34 $\pm$ 0.87 &  18.62 $\pm$ 1.90 &  9.68 $\pm$ 0.75 &  12.00 $\pm$ 1.07 &  1.55 $\pm$ 0.52     \\
              & $\text{245}\times10^3$ &  [2143680, 1745568, 2388672] & [140, 114, 156] &   8.07 $\pm$ 0.58 &  13.83 $\pm$ 0.98 &  7.68 $\pm$ 0.56 &   9.40 $\pm$ 0.77 &  1.06 $\pm$ 0.19     \\
              & $\text{490}\times10^3$ &  [3920000, 4471250, 4042500] & [128, 146, 132] &   6.89 $\pm$ 1.06 &  12.00 $\pm$ 1.80 &  6.49 $\pm$ 1.10 &   8.25 $\pm$ 1.14 &  0.87 $\pm$ 0.44     \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:scratch_results_ood_mpii}
\end{table}


==> tables/table_scratch_ood_och_results.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\caption{\textbf{Keypoint Metrics for Models Trained from Scratch - OOD Occluded Humans.}
}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{lrrrccccc}
\toprule
              dataset &     dataset size &                         training steps & no. of epochs &               AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$                \\
\midrule
COCO & 641 &                         5280 &              132 &             6.42 &             23.87 &             1.24 &             6.60 &             0.40 \\
      & 6411 &                       168252 &               84 &            19.62 &             41.28 &            16.09 &            20.51 &             2.20 \\
      & 32057 &                        40000 &              100 &            26.60 &             46.01 &            26.48 &            27.86 &             1.13 \\
      & 64115 &                       577008 &              144 &            30.34 &             49.32 &            31.08 &            31.62 &             1.54 \\\\
Synth & $\text{4.9}\times10^3$ &        [38556, 53244, 38556] &  [126, 174, 126] &  1.78 $\pm$ 0.33 &   6.26 $\pm$ 0.87 &  0.58 $\pm$ 0.12 &  2.36 $\pm$ 0.28 &  0.11 $\pm$ 0.11 \\
      & $\text{49}\times10^3$ &     [391936, 594028, 398060] &  [128, 194, 130] &  3.25 $\pm$ 0.08 &  11.09 $\pm$ 0.43 &  1.13 $\pm$ 0.06 &  3.57 $\pm$ 0.04 &  0.01 $\pm$ 0.01 \\
      & $\text{245}\times10^3$ &  [2143680, 1745568, 2388672] &  [140, 114, 156] &  2.26 $\pm$ 0.24 &   7.13 $\pm$ 0.27 &  0.89 $\pm$ 0.31 &  2.44 $\pm$ 0.22 &  0.00 $\pm$ 0.00 \\
      & $\text{490}\times10^3$ &  [3920000, 4471250, 4042500] &  [128, 146, 132] &  1.92 $\pm$ 0.41 &   5.95 $\pm$ 1.51 &  0.94 $\pm$ 0.20 &  2.11 $\pm$ 0.44 &  0.00 $\pm$ 0.00 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:scratch_results_ood_och}
\end{table}


==> tables/table_transfer_ood_crowdpose_results.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\caption{\textbf{Keypoint Metrics for Transfer-Learning Models - OOD Crowdpose Trainval.}}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{rrrrccccc}
\toprule
      real data size &     pre-training data &               training steps & no. of epochs &                AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$                \\
\midrule
641 & - &                      5280 &              132 &              9.12 &             27.58 &              4.14 &              9.97 &              6.49 \\
      & ImageNet &                      6480 &              162 &             23.82 &             53.67 &             18.02 &             26.07 &             16.49 \\
      & $\text{4.9}\times10^3$ synth &        [2960, 2240, 3840] &     [74, 56, 96] &  26.49 $\pm$ 0.73 &  54.55 $\pm$ 1.18 &  22.11 $\pm$ 0.63 &  28.91 $\pm$ 0.88 &  18.94 $\pm$ 0.53 \\
      & $\text{49}\times10^3$ synth &          [880, 720, 2480] &     [22, 18, 62] &  42.68 $\pm$ 1.60 &  70.02 $\pm$ 1.40 &  41.83 $\pm$ 1.94 &  46.07 $\pm$ 1.73 &  31.79 $\pm$ 1.41 \\
      & $\text{245}\times10^3$ synth &          [1040, 960, 800] &     [26, 24, 20] &  47.69 $\pm$ 0.25 &  74.14 $\pm$ 0.14 &  47.98 $\pm$ 0.33 &  51.30 $\pm$ 0.29 &  36.15 $\pm$ 0.16 \\
      & $\text{490}\times10^3$ synth &        [1040, 2240, 1120] &     [26, 56, 28] &  45.83 $\pm$ 3.05 &  72.41 $\pm$ 2.42 &  45.55 $\pm$ 3.61 &  49.46 $\pm$ 3.17 &  34.09 $\pm$ 2.54 \\\\
6411 & - &                     40000 &              100 &             41.78 &             70.83 &             40.57 &             44.92 &             31.17 \\
      & ImageNet &                     36800 &               92 &             48.33 &             75.58 &             48.69 &             51.98 &             35.14 \\
      & $\text{4.9}\times10^3$ synth &     [27200, 15200, 21600] &     [68, 38, 54] &  46.95 $\pm$ 0.44 &  74.15 $\pm$ 0.45 &  47.27 $\pm$ 0.61 &  50.37 $\pm$ 0.41 &  35.00 $\pm$ 0.56 \\
      & $\text{49}\times10^3$ synth &     [13600, 13600, 14400] &     [34, 34, 36] &  55.43 $\pm$ 0.34 &  79.62 $\pm$ 0.28 &  57.71 $\pm$ 0.40 &  59.16 $\pm$ 0.38 &  42.10 $\pm$ 0.42 \\
      & $\text{245}\times10^3$ synth &     [16000, 13600, 16000] &     [40, 34, 40] &  56.80 $\pm$ 0.24 &  80.35 $\pm$ 0.09 &  59.38 $\pm$ 0.25 &  60.62 $\pm$ 0.20 &  42.85 $\pm$ 0.46 \\
      & $\text{490}\times10^3$ synth &     [12800, 12800, 13600] &     [32, 32, 34] &  56.99 $\pm$ 0.56 &  80.77 $\pm$ 0.39 &  59.73 $\pm$ 0.69 &  60.84 $\pm$ 0.54 &  43.13 $\pm$ 0.74 \\\\
32057 & - &                    168252 &               84 &             62.44 &             84.22 &             65.91 &             65.97 &             49.13 \\
      & ImageNet &                    160240 &               80 &             64.15 &             85.22 &             67.72 &             67.69 &             50.33 \\
      & $\text{4.9}\times10^3$ synth &  [168252, 184276, 200300] &    [84, 92, 100] &  63.59 $\pm$ 0.08 &  85.16 $\pm$ 0.08 &  67.03 $\pm$ 0.15 &  66.93 $\pm$ 0.12 &  50.49 $\pm$ 0.31 \\
      & $\text{49}\times10^3$ synth &   [100150, 96144, 100150] &     [50, 48, 50] &  65.53 $\pm$ 0.15 &  85.93 $\pm$ 0.24 &  69.29 $\pm$ 0.14 &  68.96 $\pm$ 0.14 &  52.17 $\pm$ 0.38 \\
      & $\text{245}\times10^3$ synth &     [64096, 68102, 68102] &     [32, 34, 34] &  66.21 $\pm$ 0.04 &  86.28 $\pm$ 0.04 &  70.17 $\pm$ 0.08 &  69.80 $\pm$ 0.07 &  52.42 $\pm$ 0.20 \\
      & $\text{490}\times10^3$ synth &    [84126, 100150, 80120] &     [42, 50, 40] &  66.29 $\pm$ 0.15 &  86.30 $\pm$ 0.16 &  70.10 $\pm$ 0.16 &  69.84 $\pm$ 0.16 &  52.62 $\pm$ 0.12 \\\\
64115 & - &                    577008 &              144 &             69.78 &             88.15 &             73.99 &             73.01 &             56.68 \\
      & ImageNet &                    352616 &               88 &             69.37 &             87.95 &             73.71 &             72.71 &             55.91 \\
      & $\text{4.9}\times10^3$ synth &  [416728, 432756, 472826] &  [104, 108, 118] &  69.79 $\pm$ 0.25 &  88.19 $\pm$ 0.11 &  74.05 $\pm$ 0.19 &  73.01 $\pm$ 0.21 &  56.85 $\pm$ 0.49 \\
      & $\text{49}\times10^3$ synth &  [384672, 400700, 376658] &    [96, 100, 94] &  70.42 $\pm$ 0.09 &  88.46 $\pm$ 0.12 &  74.69 $\pm$ 0.29 &  73.59 $\pm$ 0.07 &  57.51 $\pm$ 0.20 \\
      & $\text{245}\times10^3$ synth &  [400700, 264462, 296518] &    [100, 66, 74] &  70.52 $\pm$ 0.23 &  88.41 $\pm$ 0.29 &  74.86 $\pm$ 0.25 &  73.75 $\pm$ 0.20 &  57.42 $\pm$ 0.33 \\
      & $\text{490}\times10^3$ synth &  [232406, 216378, 248434] &     [58, 54, 62] &  70.30 $\pm$ 0.06 &  88.21 $\pm$ 0.07 &  74.67 $\pm$ 0.11 &  73.55 $\pm$ 0.08 &  57.25 $\pm$ 0.17 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:transfer_results_ood_crowdpose}
\end{table}


==> tables/table_transfer_ood_lspet_results.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\caption{\textbf{Keypoint Metrics for Transfer-Learning Models - OOD Leeds Sports.}}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{rrrrccccc}
\toprule
      real data size &     pre-training data &               training steps & no. of epochs &                AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$                \\
\midrule
641 & - &                      5280 &              132 &              1.19 &              4.43 &              0.33 &              2.51 &              0.62 \\
      & ImageNet &                      6480 &              162 &              2.37 &              6.36 &              1.39 &              6.19 &              1.15 \\
      & $\text{4.9}\times10^3$ &        [2960, 2240, 3840] &     [74, 56, 96] &   3.90 $\pm$ 0.28 &   9.58 $\pm$ 0.46 &   2.61 $\pm$ 0.35 &   9.30 $\pm$ 0.45 &   1.75 $\pm$ 0.29 \\
      & $\text{49}\times10^3$ &          [880, 720, 2480] &     [22, 18, 62] &   8.37 $\pm$ 1.07 &  16.78 $\pm$ 1.85 &   7.11 $\pm$ 1.06 &  16.94 $\pm$ 1.35 &   3.13 $\pm$ 0.21 \\
      & $\text{245}\times10^3$ &          [1040, 960, 800] &     [26, 24, 20] &  11.23 $\pm$ 0.29 &  20.88 $\pm$ 0.48 &  10.18 $\pm$ 0.28 &  20.96 $\pm$ 0.48 &   3.67 $\pm$ 0.41 \\
      & $\text{490}\times10^3$ &        [1040, 2240, 1120] &     [26, 56, 28] &  10.81 $\pm$ 1.97 &  20.14 $\pm$ 2.83 &   9.64 $\pm$ 2.08 &  20.31 $\pm$ 2.74 &   3.81 $\pm$ 0.86 \\\\
6411 & - &                     40000 &              100 &              8.36 &             17.37 &              6.63 &             15.99 &              3.77 \\
      & ImageNet &                     36800 &               92 &             11.79 &             22.00 &             10.92 &             20.43 &              5.06 \\
      & $\text{4.9}\times10^3$ &     [27200, 15200, 21600] &     [68, 38, 54] &  11.10 $\pm$ 0.55 &  21.16 $\pm$ 0.99 &   9.97 $\pm$ 0.48 &  19.30 $\pm$ 0.46 &   5.24 $\pm$ 0.28 \\
      & $\text{49}\times10^3$ &     [13600, 13600, 14400] &     [34, 34, 36] &  16.54 $\pm$ 0.48 &  28.86 $\pm$ 0.85 &  15.94 $\pm$ 0.56 &  26.12 $\pm$ 0.50 &   7.83 $\pm$ 0.39 \\
      & $\text{245}\times10^3$ &     [16000, 13600, 16000] &     [40, 34, 40] &  17.40 $\pm$ 0.27 &  29.70 $\pm$ 0.28 &  16.74 $\pm$ 0.45 &  27.46 $\pm$ 0.56 &   7.91 $\pm$ 0.30 \\
      & $\text{490}\times10^3$ &     [12800, 12800, 13600] &     [32, 32, 34] &  18.16 $\pm$ 0.32 &  30.48 $\pm$ 0.54 &  17.92 $\pm$ 0.25 &  28.43 $\pm$ 0.69 &   8.71 $\pm$ 0.33 \\\\
32057 & - &                    168252 &               84 &             18.43 &             30.72 &             18.22 &             29.24 &              8.73 \\
      & ImageNet &                    160240 &               80 &             22.15 &             35.91 &             21.83 &             32.15 &             10.95 \\
      & $\text{4.9}\times10^3$ &  [168252, 184276, 200300] &    [84, 92, 100] &  20.52 $\pm$ 0.46 &  34.04 $\pm$ 0.62 &  20.25 $\pm$ 0.64 &  30.33 $\pm$ 0.24 &  10.88 $\pm$ 0.78 \\
      & $\text{49}\times10^3$ &   [100150, 96144, 100150] &     [50, 48, 50] &  24.15 $\pm$ 0.95 &  38.90 $\pm$ 1.53 &  24.14 $\pm$ 0.87 &  34.87 $\pm$ 0.67 &  12.62 $\pm$ 0.86 \\
      & $\text{245}\times10^3$ &     [64096, 68102, 68102] &     [32, 34, 34] &  25.13 $\pm$ 0.43 &  39.95 $\pm$ 0.61 &  25.06 $\pm$ 0.52 &  36.53 $\pm$ 0.21 &  12.83 $\pm$ 0.40 \\
      & $\text{490}\times10^3$ &    [84126, 100150, 80120] &     [42, 50, 40] &  24.77 $\pm$ 0.60 &  39.48 $\pm$ 0.71 &  24.61 $\pm$ 0.72 &  36.33 $\pm$ 0.90 &  12.78 $\pm$ 0.89 \\\\
64115 & - &                    577008 &              144 &             26.69 &             41.62 &             26.82 &             37.95 &             14.12 \\
      & ImageNet &                    352616 &               88 &             27.78 &             42.94 &             28.14 &             39.32 &             14.60 \\
      & $\text{4.9}\times10^3$ &  [416728, 432756, 472826] &  [104, 108, 118] &  26.41 $\pm$ 0.51 &  41.57 $\pm$ 1.12 &  26.52 $\pm$ 0.47 &  37.71 $\pm$ 0.36 &  14.18 $\pm$ 0.97 \\
      & $\text{49}\times10^3$ &  [384672, 400700, 376658] &    [96, 100, 94] &  28.34 $\pm$ 0.44 &  44.20 $\pm$ 0.48 &  28.45 $\pm$ 0.49 &  39.62 $\pm$ 0.23 &  15.03 $\pm$ 0.55 \\
      & $\text{245}\times10^3$ &  [400700, 264462, 296518] &    [100, 66, 74] &  29.61 $\pm$ 0.74 &  45.82 $\pm$ 0.89 &  29.85 $\pm$ 1.04 &  41.08 $\pm$ 0.68 &  15.76 $\pm$ 0.82 \\
      & $\text{490}\times10^3$ &  [232406, 216378, 248434] &     [58, 54, 62] &  29.58 $\pm$ 0.77 &  45.31 $\pm$ 1.26 &  29.92 $\pm$ 0.74 &  42.01 $\pm$ 0.20 &  15.53 $\pm$ 1.04 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:transfer_results_ood_lspet}
\end{table}


==> tables/table_transfer_ood_mpii_results.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\caption{\textbf{Keypoint Metrics for Transfer-Learning Models - OOD MPII Train.}}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{rrrrccccc}
\toprule
      real data size &     pre-training data &               training steps & no. of epochs &                AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$                \\
\midrule
641 & - &                      5280 & 132 &             13.99 &             37.63 &              7.90 &             14.62 &              1.24      \\
 & ImageNet &                      6480 & 162 &             31.04 &             61.58 &             26.49 &             32.81 &              3.83      \\
      & $\text{4.9}\times10^3$ synth &        [2960, 2240, 3840] & [74, 56, 96] &  36.30 $\pm$ 0.24 &  65.50 $\pm$ 0.58 &  33.78 $\pm$ 0.37 &  37.87 $\pm$ 0.31 &   8.11 $\pm$ 0.55      \\
      & $\text{49}\times10^3$ synth &          [880, 720, 2480] & [22, 18, 62] &  52.03 $\pm$ 1.85 &  76.10 $\pm$ 1.13 &  54.28 $\pm$ 2.29 &  54.07 $\pm$ 1.79 &   8.55 $\pm$ 0.51      \\
      & $\text{245}\times10^3$ synth &          [1040, 960, 800] & [26, 24, 20] &  56.27 $\pm$ 0.23 &  78.69 $\pm$ 0.27 &  59.63 $\pm$ 0.38 &  58.15 $\pm$ 0.18 &  12.23 $\pm$ 1.52      \\
      & $\text{490}\times10^3$ synth &        [1040, 2240, 1120] & [26, 56, 28] &  54.55 $\pm$ 3.17 &  77.58 $\pm$ 1.91 &  57.55 $\pm$ 3.77 &  56.55 $\pm$ 3.11 &   9.89 $\pm$ 0.86      \\\\
6411 & - &                     40000 & 100 &             48.66 &             76.69 &             49.54 &             50.40 &              4.71      \\
 & ImageNet &                     36800 & 92 &             56.61 &             82.28 &             59.65 &             58.00 &              7.67      \\
      & $\text{4.9}\times10^3$ synth &     [27200, 15200, 21600] & [68, 38, 54] &  55.55 $\pm$ 0.61 &  81.16 $\pm$ 0.50 &  58.61 $\pm$ 0.69 &  57.04 $\pm$ 0.57 &   8.85 $\pm$ 0.45      \\
      & $\text{49}\times10^3$ synth &     [13600, 13600, 14400] & [34, 34, 36] &  62.89 $\pm$ 0.11 &  84.40 $\pm$ 0.28 &  67.89 $\pm$ 0.17 &  64.40 $\pm$ 0.20 &  11.75 $\pm$ 0.78      \\
      & $\text{245}\times10^3$ synth &     [16000, 13600, 16000] & [40, 34, 40] &  63.82 $\pm$ 0.40 &  84.44 $\pm$ 0.15 &  68.98 $\pm$ 0.55 &  65.43 $\pm$ 0.37 &  11.22 $\pm$ 0.87      \\
      & $\text{490}\times10^3$ synth &     [12800, 12800, 13600] & [32, 32, 34] &  64.32 $\pm$ 0.70 &  84.99 $\pm$ 0.42 &  69.74 $\pm$ 0.88 &  65.88 $\pm$ 0.56 &  10.28 $\pm$ 1.92      \\\\
32057 & - &                    168252 & 84 &             66.86 &             86.97 &             72.77 &             68.27 &              8.65      \\
 & ImageNet &                    160240 & 80 &             68.37 &             87.83 &             74.31 &             69.65 &              9.26      \\
      & $\text{4.9}\times10^3$ synth &  [168252, 184276, 200300] & [84, 92, 100] &  66.99 $\pm$ 0.26 &  87.42 $\pm$ 0.29 &  72.59 $\pm$ 0.21 &  68.35 $\pm$ 0.23 &   8.96 $\pm$ 1.29      \\
      & $\text{49}\times10^3$ synth &   [100150, 96144, 100150] & [50, 48, 50] &  69.80 $\pm$ 0.35 &  88.25 $\pm$ 0.20 &  76.06 $\pm$ 0.51 &  71.18 $\pm$ 0.32 &  11.21 $\pm$ 0.93      \\
      & $\text{245}\times10^3$ synth &     [64096, 68102, 68102] & [32, 34, 34] &  70.55 $\pm$ 0.05 &  88.37 $\pm$ 0.16 &  76.60 $\pm$ 0.10 &  71.94 $\pm$ 0.07 &  11.67 $\pm$ 0.32      \\
      & $\text{490}\times10^3$ synth &    [84126, 100150, 80120] & [42, 50, 40] &  70.31 $\pm$  0.70 &  88.09 $\pm$  0.47 &  76.58 $\pm$  0.77 &  71.80 $\pm$  0.61 &  11.13 $\pm$  0.69      \\\\
64115 & - &                    577008 & 144 &             71.85 &             89.36 &             78.22 &             73.17 &             10.53      \\
 & ImageNet &                    352616 & 88 &             72.34 &             89.72 &             78.50 &             73.50 &             14.01      \\
      & $\text{4.9}\times10^3$ synth &  [416728, 432756, 472826] & [104, 108, 118] &  71.93 $\pm$ 0.08 &  89.45 $\pm$ 0.27 &  78.37 $\pm$ 0.11 &  73.15 $\pm$ 0.08 &  11.21 $\pm$ 0.67      \\
      & $\text{49}\times10^3$ synth &  [384672, 400700, 376658] & [96, 100, 94] &  72.44 $\pm$ 0.13 &  89.56 $\pm$ 0.18 &  79.03 $\pm$ 0.08 &  73.66 $\pm$ 0.10 &  11.46 $\pm$ 0.77      \\
      & $\text{245}\times10^3$ synth &  [400700, 264462, 296518] & [100, 66, 74] &  72.71 $\pm$ 0.28 &  89.38 $\pm$ 0.19 &  79.20 $\pm$ 0.32 &  74.05 $\pm$ 0.22 &  11.79 $\pm$ 0.12      \\
      & $\text{490}\times10^3$ synth &  [232406, 216378, 248434] & [58, 54, 62] &  72.77 $\pm$ 0.17 &  89.28 $\pm$ 0.24 &  79.19 $\pm$ 0.09 &  74.11 $\pm$ 0.10 &  11.28 $\pm$ 0.33      \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:transfer_results_ood_mpii}
\end{table}


==> tables/table_transfer_ood_och_results.tex <==
% ===============================================================================================
% ====================================== NEW RESULTS ============================================
% ===============================================================================================
\begin{table}[htb]
\caption{\textbf{Keypoint Metrics for Transfer-Learning Models - OOD Occluded Humans.}}
\begin{adjustbox}{max width=\textwidth}
\centering
\begin{tabular}{rrrrccccc}
\toprule
      real data size &     pre-training data &               training steps & no. of epochs &                AP &              $\textrm{AP}^{\textrm{\textit{IoU=.50}}}$ &             $\textrm{AP}^{\textrm{\textit{IoU=.75}}}$ &               $\textrm{AP}^{\textrm{\textit{large}}}$ &              $\textrm{AP}^{\textrm{\textit{medium}}}$                \\
\midrule
641 & - &                      5280 &              132 &              6.42 &             23.87 &              1.24 &              6.60 &              0.40 \\
      & ImageNet &                      6480 &              162 &             14.00 &             38.42 &              6.74 &             14.51 &              1.31 \\
      & $\text{4.9}\times10^3$ &        [2960, 2240, 3840] &     [74, 56, 96] &  13.68 $\pm$ 0.28 &  36.51 $\pm$ 0.60 &   7.49 $\pm$ 0.16 &  14.29 $\pm$ 0.35 &   1.35 $\pm$ 0.44 \\
      & $\text{49}\times10^3$ &          [880, 720, 2480] &     [22, 18, 62] &  20.01 $\pm$ 1.21 &  43.35 $\pm$ 1.66 &  15.56 $\pm$ 1.35 &  20.92 $\pm$ 1.18 &  11.92 $\pm$ 5.48 \\
      & $\text{245}\times10^3$ &          [1040, 960, 800] &     [26, 24, 20] &  22.70 $\pm$ 0.14 &  45.49 $\pm$ 0.19 &  19.53 $\pm$ 0.37 &  23.73 $\pm$ 0.17 &   6.08 $\pm$ 2.06 \\
      & $\text{490}\times10^3$ &        [1040, 2240, 1120] &     [26, 56, 28] &  21.26 $\pm$ 1.19 &  43.46 $\pm$ 1.47 &  17.76 $\pm$ 1.68 &  22.40 $\pm$ 1.26 &  11.61 $\pm$ 5.34 \\\\
6411 & - &                     40000 &              100 &             19.62 &             41.28 &             16.09 &             20.51 &              2.20 \\
      & ImageNet &                     36800 &               92 &             21.58 &             42.46 &             18.91 &             22.67 &              1.02 \\
      & $\text{4.9}\times10^3$ &     [27200, 15200, 21600] &     [68, 38, 54] &  20.99 $\pm$ 0.19 &  42.45 $\pm$ 0.23 &  17.87 $\pm$ 0.27 &  21.93 $\pm$ 0.19 &   4.80 $\pm$ 0.56 \\
      & $\text{49}\times10^3$ &     [13600, 13600, 14400] &     [34, 34, 36] &  24.57 $\pm$ 0.05 &  45.01 $\pm$ 0.20 &  23.12 $\pm$ 0.20 &  25.66 $\pm$ 0.07 &   4.29 $\pm$ 2.41 \\
      & $\text{245}\times10^3$ &     [16000, 13600, 16000] &     [40, 34, 40] &  25.32 $\pm$ 0.41 &  45.31 $\pm$ 0.36 &  24.54 $\pm$ 0.56 &  26.42 $\pm$ 0.39 &   2.33 $\pm$ 0.85 \\
      & $\text{490}\times10^3$ &     [12800, 12800, 13600] &     [32, 32, 34] &  25.71 $\pm$ 0.38 &  45.77 $\pm$ 0.60 &  24.90 $\pm$ 0.46 &  26.77 $\pm$ 0.36 &   3.27 $\pm$ 0.24 \\\\
32057 & - &                    168252 &               84 &             26.60 &             46.01 &             26.48 &             27.86 &              1.13 \\
      & ImageNet &                    160240 &               80 &             27.61 &             47.28 &             27.76 &             28.87 &              1.20 \\
      & $\text{4.9}\times10^3$ &  [168252, 184276, 200300] &    [84, 92, 100] &  27.72 $\pm$ 0.04 &  47.25 $\pm$ 0.09 &  27.53 $\pm$ 0.24 &  28.92 $\pm$ 0.05 &   2.26 $\pm$ 0.88 \\
      & $\text{49}\times10^3$ &   [100150, 96144, 100150] &     [50, 48, 50] &  29.01 $\pm$ 0.44 &  48.28 $\pm$ 0.62 &  29.32 $\pm$ 0.53 &  30.20 $\pm$ 0.40 &   6.37 $\pm$ 5.35 \\
      & $\text{245}\times10^3$ &     [64096, 68102, 68102] &     [32, 34, 34] &  29.52 $\pm$ 0.17 &  48.53 $\pm$ 0.28 &  30.33 $\pm$ 0.20 &  30.76 $\pm$ 0.14 &   3.04 $\pm$ 0.91 \\
      & $\text{490}\times10^3$ &    [84126, 100150, 80120] &     [42, 50, 40] &  29.51 $\pm$ 0.08 &  48.43 $\pm$ 0.27 &  30.39 $\pm$ 0.09 &  30.75 $\pm$ 0.05 &   1.83 $\pm$ 0.16 \\\\
64115 & - &                    577008 &              144 &             30.34 &             49.32 &             31.08 &             31.62 &              1.54 \\
      & ImageNet &                    352616 &               88 &             30.68 &             49.98 &             31.66 &             31.90 &              5.22 \\
      & $\text{4.9}\times10^3$ &  [416728, 432756, 472826] &  [104, 108, 118] &  30.65 $\pm$ 0.27 &  49.39 $\pm$ 0.08 &  31.67 $\pm$ 0.38 &  31.87 $\pm$ 0.24 &   5.30 $\pm$ 4.21 \\
      & $\text{49}\times10^3$ &  [384672, 400700, 376658] &    [96, 100, 94] &  30.79 $\pm$ 0.41 &  49.43 $\pm$ 0.51 &  32.06 $\pm$ 0.57 &  32.03 $\pm$ 0.37 &   3.67 $\pm$ 0.94 \\
      & $\text{245}\times10^3$ &  [400700, 264462, 296518] &    [100, 66, 74] &  31.34 $\pm$ 0.50 &  49.81 $\pm$ 0.54 &  32.92 $\pm$ 0.71 &  32.62 $\pm$ 0.46 &   6.94 $\pm$ 6.58 \\
      & $\text{490}\times10^3$ &  [232406, 216378, 248434] &     [58, 54, 62] &  31.34 $\pm$ 0.25 &  49.93 $\pm$ 0.41 &  32.83 $\pm$ 0.34 &  32.65 $\pm$ 0.22 &   2.47 $\pm$ 1.04 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:transfer_results_ood_och}
\end{table}

